Performance-Aware Self-Configurable Multi-Agent Networks: A Distributed Submodular Approach for Simultaneous Coordination and Network Design

We introduce the first, to our knowledge, rigorous approach that enables multi-agent networks to self-configure their communication topology to balance the trade-off between scalability and optimality during multi-agent planning. We are motivated by the future of ubiquitous collaborative autonomy where numerous distributed agents will be coordinating via agent-to-agent communication to execute complex tasks such as traffic monitoring, event detection, and environmental exploration. But the explosion of information in such large-scale networks currently curtails their deployment due to impractical decision times induced by the computational and communication requirements of the existing near-optimal coordination algorithms. To overcome this challenge, we present the AlterNAting COordination and Network-Design Algorithm (Anaconda), a scalable algorithm that also enjoys near-optimality guarantees. Subject to the agents' bandwidth constraints, Anaconda enables the agents to optimize their local communication neighborhoods such that the action-coordination approximation performance of the network is maximized. Compared to the state of the art, Anaconda is an anytime self-configurable algorithm that quantifies its suboptimality guarantee for any type of network, from fully disconnected to fully centralized, and that, for sparse networks, is one order faster in terms of decision speed. To develop the algorithm, we quantify the suboptimality cost due to decentralization, i.e., due to communication-minimal distributed coordination. We also employ tools inspired by the literature on multi-armed bandits and submodular maximization subject to cardinality constraints. We demonstrate Anaconda in simulated scenarios of area monitoring and compare it with a state-of-the-art algorithm.

==> alg-EXP3-IX.tex <==
\setlength{\textfloatsep}{3mm}
\begin{algorithm}[t]
	\caption{\expthreeix~\cite{neu2015explore}
	}\label{alg:expthreeix}
	\begin{algorithmic}[1]
		\REQUIRE Number of time steps $T$ and ground set $\calV$.
		\ENSURE Probability distribution $z_t \myin \{[0,1]^{|\calV|}:\|z_t \|_1=$ $1\}$ over $\calV$ at each $t\in[T]$.
		\smallskip
		
		\STATE $\eta\gets\sqrt{2\log{|\calV|}\,/\,{(|\calV|T)}}$; $\gamma=\eta/2$;
		\STATE $w_{1}\gets\left[w_{1,\,1}, \dots, w_{|\calV|,\,1}\right]^\top$ with $w_{v,\,1}=1, \forall v\in \calV$;
        \FOR {each time step $t\in[T]$}
        \STATE \textbf{output} $z_t\gets{w_t}\,/\,{\|w_t\|_1}$;
        \STATE \textbf{receive} reward $r_{v_t,\,t}\in [0,1]$ of selecting $v_t\in\calV$ at $t$; 
        \STATE $\Tilde{r}_{v,\,t} \gets 1 - \frac{{\bf 1}(v_t\,=\,v)}{z_{v,t}\,+\,\gamma}(1\,-\,r_{v_t,\,t})$, for all $v\in\calV$;
        \STATE $w_{v,\,t+1}\gets w_{v,\,t}\exp{(\eta \,\Tilde{r}_{v,\,t})}$, for all $v\in\calV$;
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

==> fig-intro.tex <==
%!TEX root = 1-Introduction.tex

\begin{figure}[t]
    \captionsetup{font=footnotesize}
    \centering
\hspace{0.4mm}\includegraphics[width=.99\columnwidth]{figures/CDC24_block_diagram.png}
    \vspace{-5mm}
    \caption{\textbf{Overview of AlterNAting COordination and Network-Design Algorithm ({\fontsize{7}{7}\selectfont\sf Anaconda})}. Starting from an unspecified communication network, and subject to the agents' communication bandwidth and connectivity constraints, {\fontsize{7}{7}\selectfont\sf Anaconda} enables the agents to optimize their local communication neighborhoods such that the action-coordination performance of the multi-agent network is optimal. To this end, {\fontsize{7}{7}\selectfont\sf Anaconda} employs two subroutines, {\fontsize{7}{7}\selectfont\sf ActionCoordination} and {\fontsize{7}{7}\selectfont\sf NeighborSelection}, that alternate optimization.  In more detail,  given the selected neighborhoods $\{\calN_i\}_{i\in\calN}$ by {\fontsize{7}{7}\selectfont\sf NeighborSelection}, {\fontsize{7}{7}\selectfont\sf ActionCoordination} instructs the agents to select actions to jointly maximize \cref{eq:intro}. But {\fontsize{7}{7}\selectfont\sf ActionCoordination} incurs a suboptimality cost $C(\{\calN_i\}_{i\in\calN})$ due to forcing the agents to coordinate exchanging local information only and prohibiting multi-hop communication in favor of decision speed.  For this reason, given the agents' bandwidth and connectivity constraints, and the previously selected actions by {\fontsize{7}{7}\selectfont\sf ActionCoordination},  {\fontsize{7}{7}\selectfont\sf NeighborSelection} instructs each agent~$i$  to design its neighborhood $\calN_i$ to optimize $C(\{\calN_i\}_{i\in\calN})$ and, thus, maximize the approximation performance of {\fontsize{7}{7}\selectfont\sf ActionCoordination} in the subsequent iteration. 
    }\label{fig:overview}
   \vspace{-7mm}
\end{figure}

==> preamble_packages.tex <==
%!TEX root = main.tex

% LC: debug
%==========================================================================
%\usepackage{refcheck}
%\usepackage[notref]{showkeys}
%==========================================================================

% LC: to be used for TRO
%==========================================================================
% \usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%==========================================================================
\usepackage{comment}
\usepackage{siunitx}
\usepackage{relsize}
\usepackage{ifthen}

\usepackage[caption=false]{subfig}

% \begin{comment}
% % Fancy formatting 
% \usepackage[tracking=false,kerning=true,spacing=true]{microtype}
% \usepackage[caption=false]{subfig}

% \usepackage[style=numeric-comp,sorting=none,firstinits=true, maxnames=3,bibstyle=numeric,abbreviate=false,defernums=true,eprint=false,backend=bibtex]{biblatex}
% \renewcommand{\bibfont}{\footnotesize}
% % \DeclareFieldFormat[article]{pages}{#1}%
% % \DeclareFieldFormat[inproceedings]{pages}{#1}%

% \AtEveryBibitem{%
%   \ifentrytype{article}{%
%     \clearfield{pages}%
%   }{%
%   }%
%   \ifentrytype{inproceedings}{%
%     \clearfield{pages}%
%   }{%
%   }%
% }
% \end{comment}

% \bibliography{commons/bib/strings_long}
% \bibliography{commons/bib/all_only_one_w_pages}
% \bibliography{../../references/references}

% \usepackage[noadjust]{cite}
%\usepackage[vlined,ruled,linesnumbered]{algcompatible}
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{rotating}
\usepackage{color}
\usepackage{enumerate}
\usepackage[T1]{fontenc}
\usepackage{psfrag}
\usepackage{epsfig} % for postscript graphics files
%\usepackage{subfigure}
% \usepackage{hyperref}
\usepackage{booktabs}
\usepackage{graphicx,url}
\usepackage{multirow}
\usepackage{array}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{xstring}
%\usepackage[noend]{algorithmic}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{prettyref}
\usepackage{flexisym}
\usepackage{bigdelim}
\usepackage{breqn} % load this last
\usepackage{listings}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{bm}
\graphicspath{{./figures/}}
\usepackage{tikz}
\usetikzlibrary{matrix,calc}


%\usepackage{amsthm} % math
\usepackage{lineno}



%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%    dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.

% *** GRAPHICS RELATED PACKAGES ***
%
%\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
%\fi


\usepackage{mdwlist}
\let\stditemize\itemize
\let\endstditemize\enditemize
\let\itemize\undefined
\makecompactlist{itemize}{stditemize}

%\let\stdenumerate\enumerate
%\let\endstdenumerate\endenumerate
%\let\enumerate\undefined
%\makecompactlist{enumerate}{stdenumerate}
 

